Machine Learning for the EUSO-SPB2 Fluorescence Telescope Data Analysis

The Extreme Universe Space Observatory on a Super Pressure Balloon 2 (EUSO-SPB2) is the most advanced balloon mission undertaken by the JEM-EUSO collaboration. EUSO-SPB2 is built on the experience of previous stratosphere missions, EUSO-Balloon and EUSO-SPB, and of the Mini-EUSO space mission currently active onboard the International Space Station. EUSO- SPB2 is equipped with two instruments: a fluorescence telescope aimed at registering ultra-high energy cosmic rays (UHECRs) with an energy above 2 EeV and a Cherenkov telescope built to measure direct Cherenkov emission from cosmic rays with energies above 1 PeV. The EUSO-SPB2 mission will provide pioneering observations on the path towards a space-based multi-messenger observatory. As such, a special attention was paid to the development of triggers and other software aimed at comprehensive data analysis. A whole number of methods based on machine learning (ML) and neural networks was developed during the construction of the experiment and a few others are under active development. Here we provide a brief review of the ML-based methods already implemented in the instrument and the ground software and report preliminary results on the ML-based reconstruction of UHECR parameters for the fluorescence telescope.

==> JEM-EUSO_Authors_July2023.tex <==
\newpage
\noindent
{\Large\bf Full Authors list: The JEM-EUSO Collaboration\\}
%{\scriptsize (author-list as of July 1st, 2023)} \hspace{0.6cm}
%{\scriptsize (version  \today{} \currenttime{})}
%\vspace*{0.5cm}

\begin{sloppypar}
{\small \noindent
S.~Abe$^{fq}$, 
J.H.~Adams Jr.$^{pd}$, 
D.~Allard$^{cb}$,
P.~Alldredge$^{pd}$,
L.~Anchordoqui$^{pe}$,
A.~Anzalone$^{eh,ed}$, 
E.~Arnone$^{ek,el}$,
M.~Bagheri$^{ph}$,
B.~Baret$^{cb}$,
D.~Barghini$^{el,ek}$,
M.~Battisti$^{ek,el,cb}$,
R.~Bellotti$^{ea,eb}$, 
A.A.~Belov$^{kb}$, 
M.~Bertaina$^{ek,el}$,
P.F.~Bertone$^{pf}$,
M.~Bianciotto$^{ek,el}$,
P.L.~Biermann$^{db}$,
F.~Bisconti$^{ei}$, 
C.~Blaksley$^{ft}$, 
S.~Blin-Bondil$^{cb}$, 
K.~Bolmgren$^{na}$,
S.~Briz$^{pb}$,
J.~Burton$^{pd}$,
F.~Cafagna$^{ea.eb}$, 
G.~Cambi\'e$^{ei,ej}$,
D.~Campana$^{ef}$, 
F.~Capel$^{de}$, 
R.~Caruso$^{ec,ed}$, 
M.~Casolino$^{ft,ei,ej}$,
C.~Cassardo$^{ek,el}$, 
A.~Castellina$^{ek,em}$,
K.~\v{C}ern\'{y}$^{bb}$,  
M.J.~Christl$^{pf}$, 
R.~Colalillo$^{ef,eg}$,
L.~Conti$^{en,ei}$, 
G.~Cotto$^{ek,el}$, 
H.J.~Crawford$^{pa}$, 
R.~Cremonini$^{el}$,
A.~Creusot$^{cb}$, 
A.~de Castro G\'onzalez$^{pb}$,  
C.~de la Taille$^{ca}$, 
R.~Diesing$^{pb}$,
P.~Dinaucourt$^{ca}$,
A.~Di Nola$^{eg}$,
A.~Ebersoldt$^{db}$,
T.~Ebisuzaki$^{ft}$,
J.~Eser$^{pb}$,
F.~Fenu$^{eo}$, 
S.~Ferrarese$^{ek,el}$,
G.~Filippatos$^{pc}$, 
W.W.~Finch$^{pc}$,
F. Flaminio$^{eg}$,
C.~Fornaro$^{en,ei}$,
D.~Fuhne$^{pc}$,
C.~Fuglesang$^{na}$, 
M.~Fukushima$^{fe}$, 
S.~Gadamsetty$^{ph}$,
D.~Gardiol$^{ek,em}$,
G.K.~Garipov$^{kb}$, 
E.~Gazda$^{ph}$, 
A.~Golzio$^{ek,el}$,
F.~Guarino$^{ef,eg}$, 
C.~Gu\'epin$^{pb}$,
A.~Haungs$^{db}$,
T.~Heibges$^{pc}$,
F.~Isgr\`o$^{ef,eg}$, 
E.G.~Judd$^{pa}$, 
F.~Kajino$^{ff}$, 
I.~Kaneko$^{ft}$, 
M.~Kleifges$^{db}$,
P.A.~Klimov$^{kb}$,
I.~Kreykenbohm$^{da}$, 
J.F.~Krizmanic$^{pj}$, 
V.~Kungel$^{pc}$,  
E.~Kuznetsov$^{pd}$, 
F.~L\'opez~Mart\'inez$^{pb}$, 
D.~Mand\'{a}t$^{bc}$,
M.~Manfrin$^{ek,el}$,
A. Marcelli$^{ej}$,
L.~Marcelli$^{ei}$, 
W.~Marsza{\l}$^{ia}$, 
J.N.~Matthews$^{pg}$, 
A.~Menshikov$^{db}$,
M.~Mese$^{ef,eg}$, 
S.S.~Meyer$^{pb}$,
J.~Mimouni$^{ad}$, 
H.~Miyamoto$^{ek,el}$, 
Y.~Mizumoto$^{fi}$,
A.~Monaco$^{ea,eb}$, 
S.~Nagataki$^{ft}$, 
J.~M.~Nachtman$^{pi}$,
D.~Naumov$^{ka}$,
A.~Neronov$^{cb}$,  
T.~Nonaka$^{fe}$, 
T.~Ogawa$^{ft}$, 
S.~Ogio$^{ft}$, 
H.~Ohmori$^{ft}$, 
A.V.~Olinto$^{pb}$,
Y.~Onel$^{pi}$,
G.~Osteria$^{ef}$,  
A.N.~Otte$^{ph}$,  
A.~Pagliaro$^{eh,ed}$,  
B.~Panico$^{ef, eg}$,  
E.~Parizot$^{cb, cd}$, 
I.H.~Park$^{gb}$, 
T.~Paul$^{pe}$,
M.~Pech$^{bc}$, 
F.~Perfetto$^{ef}$,  
P.~Picozza$^{ei,ej}$, 
L.W.~Piotrowski$^{ib}$,
Z.~Plebaniak$^{ei, ej}$, 
J.~Posligua$^{pi}$,
M.~Potts$^{ph}$,
R.~Prevete$^{ef,eg}$,
G.~Pr\'ev\^ot$^{cb}$,
M.~Przybylak$^{ia}$, 
E.~Reali$^{ei, ej}$,
P.~Reardon$^{pd}$, 
M.H.~Reno$^{pi}$, 
M.~Ricci$^{ee}$, 
O.F.~Romero~Matamala$^{ph}$, 
G.~Romoli$^{ei, ej}$,
H.~Sagawa$^{fe}$, 
N.~Sakaki$^{ft}$, 
A.~Santangelo$^{dd}$, 
O.A.~Saprykin$^{kc}$,
F.~Sarazin$^{pc}$,
M.~Sato$^{fo}$, 
H.~Schieler$^{db}$,
P.~Schov\'{a}nek$^{bc}$,
V.~Scotti$^{ef,eg}$,
S.~Selmane$^{cb}$
S.A.~Sharakin$^{kb}$,
K.~Shinozaki$^{ia}$, 
S.~Stepanoff$^{ph}$,
J.F.~Soriano$^{pe}$,
J.~Szabelski$^{ia}$,
N.~Tajima$^{ft}$, 
T.~Tajima$^{ft, pn}$,
Y.~Takahashi$^{fo}$, 
M.~Takeda$^{fe}$, 
Y.~Takizawa$^{ft}$, 
C.~Tenzer$^{dd}$,
S.B.~Thomas$^{pg}$, 
L.G.~Tkachev$^{ka}$,
T.~Tomida$^{fh}$, 
S.~Toscano$^{ob}$,  
M.~Tra\"{i}che$^{aa}$,  
D.~Trofimov$^{cb,kb}$,
K.~Tsuno$^{ft}$,  
P.~Vallania$^{ek,em}$,
L.~Valore$^{ef,eg}$,
T.~M.~Venters$^{pj}$,
C.~Vigorito$^{ek,el}$, 
M.~Vrabel$^{ia}$, 
S.~Wada$^{ft}$,  
J.~Watts~Jr.$^{pd}$, 
A.~Weindl$^{db}$,
L.~Wiencke$^{pc}$, 
J.~Wilms$^{da}$,
D.~Winn$^{pm}$,
H.~Wistrand$^{pc}$,
I.V.~Yashin$^{kb}$, 
R.~Young$^{pf}$,
M.Yu.~Zotov$^{kb}$.
}
\end{sloppypar}
\vspace*{.3cm}

%%\newpage
{ \footnotesize
\noindent
% Algeria - 2 institutes
$^{aa}$ Centre for Development of Advanced Technologies (CDTA), Algiers, Algeria \\
$^{ad}$ Lab. of Math. and Sub-Atomic Phys. (LPMPS), Univ. Constantine I, Constantine, Algeria \\
% Czech Republic - 2 institutes
$^{bb}$ Joint Laboratory of Optics, Faculty of Science, Palack\'{y} University, Olomouc, Czech Republic\\
$^{bc}$ Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic\\
% France - 3 institutes  
$^{ca}$ Omega, Ecole Polytechnique, CNRS/IN2P3, Palaiseau, France\\
$^{cb}$ Universit\'e de Paris, CNRS, AstroParticule et Cosmologie, F-75013 Paris, France\\
$^{cd}$ Institut universitaire de France (IUF)\\
% Germany - 4 institutes
$^{da}$ ECAP, University of Erlangen-Nuremberg, Germany\\
$^{db}$ Karlsruhe Institute of Technology (KIT), Germany\\
$^{dd}$ Institute for Astronomy and Astrophysics, Kepler Center, University of T\"ubingen, Germany\\
$^{de}$ Max Planck Institute for Physics, Munich, Germany\\
% Italy - 15 institutes  
$^{ea}$ Istituto Nazionale di Fisica Nucleare - Sezione di Bari, Italy\\
$^{eb}$ Universita' degli Studi di Bari Aldo Moro and INFN - Sezione di Bari, Italy\\
$^{ec}$ Dipartimento di Fisica e Astronomia "Ettore Majorana", Universita' di Catania, Italy\\
$^{ed}$ Istituto Nazionale di Fisica Nucleare - Sezione di Catania, Italy\\
$^{ee}$ Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, Italy\\
$^{ef}$ Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Italy\\
$^{eg}$ Universita' di Napoli Federico II - Dipartimento di Fisica "Ettore Pancini", Italy\\
$^{eh}$ INAF - Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy\\
$^{ei}$ Istituto Nazionale di Fisica Nucleare - Sezione di Roma Tor Vergata, Italy\\
$^{ej}$ Universita' di Roma Tor Vergata - Dipartimento di Fisica, Roma, Italy\\
$^{ek}$ Istituto Nazionale di Fisica Nucleare - Sezione di Torino, Italy\\
$^{el}$ Dipartimento di Fisica, Universita' di Torino, Italy\\
$^{em}$ Osservatorio Astrofisico di Torino, Istituto Nazionale di Astrofisica, Italy\\
$^{en}$ Uninettuno University, Rome, Italy\\
$^{eo}$ Agenzia Spaziale Italiana, Via del Politecnico, 00133, Roma, Italy\\
% Japan - 7 institutes 
$^{fe}$ Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Japan\\ 
$^{ff}$ Konan University, Kobe, Japan\\ 
$^{fh}$ Shinshu University, Nagano, Japan \\
$^{fi}$ National Astronomical Observatory, Mitaka, Japan\\ 
$^{fo}$ Hokkaido University, Sapporo, Japan \\ 
$^{fq}$ Nihon University Chiyoda, Tokyo, Japan\\ 
$^{ft}$ RIKEN, Wako, Japan\\
% Korea - 1 institute
$^{gb}$ Sungkyunkwan University, Seoul, Republic of Korea\\
% Poland - 2 institutes
$^{ia}$ National Centre for Nuclear Research, Otwock, Poland\\
$^{ib}$ Faculty of Physics, University of Warsaw, Poland\\
% Russia - 3 institutes 
$^{ka}$ Joint Institute for Nuclear Research, Dubna, Russia\\
$^{kb}$ Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Russia\\
$^{kc}$ Space Regatta Consortium, Korolev, Russia\\
% Sweden - 1 institute 
$^{na}$ KTH Royal Institute of Technology, Stockholm, Sweden\\
% Switzerland - 1 institute 
$^{ob}$ ISDC Data Centre for Astrophysics, Versoix, Switzerland\\
% USA - 12 institutes 
$^{pa}$ Space Science Laboratory, University of California, Berkeley, CA, USA\\
$^{pb}$ University of Chicago, IL, USA\\
$^{pc}$ Colorado School of Mines, Golden, CO, USA\\
$^{pd}$ University of Alabama in Huntsville, Huntsville, AL; USA\\
$^{pe}$ Lehman College, City University of New York (CUNY), NY, USA\\
$^{pf}$ NASA Marshall Space Flight Center, Huntsville, AL, USA\\
$^{pg}$ University of Utah, Salt Lake City, UT, USA\\
$^{ph}$ Georgia Institute of Technology, USA\\
$^{pi}$ University of Iowa, Iowa City, IA, USA\\
$^{pj}$ NASA Goddard Space Flight Center, Greenbelt, MD, USA\\
$^{pm}$ Fairfield University, Fairfield, CT, USA\\
$^{pn}$ Department of Physics and Astronomy, University of California, Irvine \\
}

